Adaptive whitening in neural populations with gain-modulating interneurons

Statistical whitening transformations play a fundamental role in many computational systems, and may also play an important role in biological sensory systems. Existing neural circuit models of adaptive whitening operate by modifying synaptic interactions; however, such modifications would seem both too slow and insufficiently reversible. Motivated by the extensive neuroscience literature on gain modulation, we propose an alternative model that adaptively whitens its responses by modulating the gains of individual neurons. Starting from a novel whitening objective, we derive an online algorithm that whitens its outputs by adjusting the marginal variances of an overcomplete set of projections. We map the algorithm onto a recurrent neural network with fixed synaptic weights and gain-modulating interneurons. We demonstrate numerically that sign-constraining the gains improves robustness of the network to ill-conditioned inputs, and a generalization of the circuit achieves a form of local whitening in convolutional populations, such as those found throughout the visual or auditory systems.

==> rebuttals.tex <==
\newcommand{\lyndon}[1]{{\color{RoyalBlue} #1}}
\newcommand{\david}[1]{{\color{RubineRed} #1}}
\newcommand{\eero}[1]{{\color{ForestGreen} #1}}
\newcommand{\mitya}[1]{{\color{Fuchsia} MC: #1}}

\section{Rebuttals}

\subsection{Reviewer 1: 7(3)}

\subsubsection{Questions}
I am wondering how authors enforce the polarity of weight during the training which is important to claim some neurons are excitatory or inhibitory.

%\eero{Feels like we are over-responding, well beyond the question being asked... I suggest simplification :)}

\david{Since the weights remain fixed throughout adaptive whitening, we only need to enforce polarity of the weights at initialization (e.g., the weights used in Figures 1 and 2 are non-negative).}
% However, in Algorithm 1, the gains are not sign-constrained during training, so the circuit can violate Dale's law. One way to address this is to enforce non-negativity of the gains by rectifying the gain update. As we show in Sec 4.4, this modification is also useful for preventing noise amplification.}


\subsubsection{Limitations}
It would be great if the author could discuss how the ZCA framework can be extended to include several major classes of inhibitory interneurons in the cortex.

\lyndon{
Thank you for the suggestion: We will include a reference (e.g., Kepecs \& Fishell 2014; Nature Review), and possible relationship to our framework. Specifically, we think our adaptive ZCA paradigm would most naturally be implemented with a single class of interneuron that has local and reciprocal connectivity to the primary/pyramidal cells (e.g. somatostatin interneurons in the cortex or granule cells in the olfactory bulb), and a modulatory gain timescale slower than the primary/pyramidal cell responses. The relative number of such neurons would determine the whitening capabilities. These are testable predictions, and we hope that our work can inspire experimentalists to look for them.
}

\subsection{Reviewer 2: 3(4)}

\subsubsection{Weaknesses}
1. While the ideas are well-communicated, I found it somewhat difficult to judge how well the algorithm performs. For example, in Figs 2-3, the Frobenius norm of the difference between $\rmC_{yy}$ and $\rmI_N$ is used to quantify the whitening of the inputs. While a norm of 0.01, attained in both figures by the algorithm, may well correspond to very good performance, we see that, in Fig. 3, optimal performance is well below 0.001. How might the readers judge the differences in the performance of the proposed algorithm vs the optimal case more concretely? Perhaps the extra performance obtained using the spectral frame results in little practical gains, for example, or perhaps the practical differences are very large. Minimally it seems that providing the resultant scatter plots, like those shown in Fig. 5, would be a good place to start. Are there other ways--e.g., perhaps a $\Vert \rmC_{yy} - \rmI_N \Vert$ threshold--to judge whether the performance is sufficient, even if it is context dependent? 


% \eero{EPS: see my coments in overleaf, regarding "metric".}
\david{Thank you for noting this point of confusion. Indeed, the difference between Frobenius error of 0.01 and 0.001 is difficult to detect in the corresponding scatter plots. As a visual indicator, we will include scatter plots as well as covariance ellipsoids throughout training. We will also include an additional evaluation criterion using the matrix operator norm:
$\Vert {\bf C}_{yy}- {\bf I}_N\Vert_{Op}$, 
which measures the largest eigenvalue of ${\bf C}_{yy}-{\bf I}_N$.
To judge whether the performance is sufficient, we will use the threshold $\|{\bf C}_{yy}-{\bf I}_N\|_{Op}\le0.1$, which measures the point at which the covariance ellipsoid's principal axes are within 0.1 of unity. Visually this means the ellipsoid corresponding to ${\bf C}_{yy}$ lies between the circles with radii 0.9 and 1.1.
}

2. While the authors emphasize that an advantage of their method is that W remains fixed for any given implementation of their algorithm, they also either do not specify or else change the choice of frame throughout the manuscript, making it difficult to synthesize a full judgment of the algorithm, especially as the authors emphasize that the choice of frame indeed affects the algorithm's performance (L 250). For the first and third experiments (Sec 4.1, 4.4), I did not find W specified. In the second experiment (4.2), both random and optimized were compared. Next (4.5), yet another frame construction choice was employed. Yet, I did not observe anywhere any guidance on how to optimally (even if heuristically) choose W. Instead, in the discussion, the authors appear to contradict themselves by saying (L 418), "Indeed, the demonstrations in this study were largely agnostic to the exact structure of the weights W." This is in direct contrast to their earlier statement (L 250, authors' emphasis), "These results indicate that the choice of frame \textit{does} in fact play an important role in the effectiveness of our algorithm."

\david{Thanks for pointing out these inconsistencies in our presentation. We'll revise to state which frame is used in each figure, and unify the text to make it clear that:
\begin{itemize}
    \item[1.] The result expressed in Proposition 2.1 is exact: the optimal solution to the whitening objective (Eq. 5) does \textit{not} depend on the choice of frame (provided Eq. 3 holds). 
    \item[2.] On the other hand, the numerical experiments indicate that the convergence rate of Algorithm 1 \textit{does} depend on the choice of frame (Sec 4.2).  Specifically, the conditioning of the basis in Eq 3 determines convergence rate.
    \item[3.] Based on numerical experiments, and assuming that the input data distribution is unknown, convergence is best for an equi-angular frame (see, e.g., Fig 5). In high dimensions, this generally must be approximated through numerical optimization.
%    If the input data distribution is known a priori, then the best frame is the spectral frame which only requires $N$ frame vectors (the eigenvectors of the covariance matrix).
\end{itemize}
%In addition to clearly stating the above points, we will also clarify which frame is used in each figure.
}

% \lyndon{Our apologies for the confusion; our phrasing was correct but imprecise, and we will amend the text to improve clarity. 
% We were mixing distinct concepts: whereas the solution to the whitening objective (Eq. 5) does \textit{not} depend on the choice of frame (assuming Eq. 3 holds), the convergence rate of the Algorithm \textit{does} depend on the frame (Sec 4.2).
% Indeed, the results of Sec 4.2 ("Rate of convergence depends on frame ${\bf W}$") were shown to illustrate a simple heuristic to choose ${\bf W}$, but we will amend the text to make this crystal clear. The heuristic and its motivation are summarized as follows. 1) We note that the best achievable algorithmic convergence is when the frame contains the eigenvectors of the inputs. However, this may be quite restrictive because it assumes the statistics of the input have already been learned, and would seem quite specialized to a single context. 2) A heuristic for choosing ${\bf W}$ when the inputs have not yet been learned is to use a frame that is optimized to splay the space (e.g. an equiangular frame), which systematically performs better than one that with purely random elements. This Optimized frame has increased probability of alignment with the eigenvectors of given inputs, and (as we know from Eqs. 3 and 5) is guaranteed to eventually converge for all possible contexts.
% This naturally leads into Sec 4.4, where we ask how the network performs if multiple contexts are pre-learned and embedded in ${\bf W}$.

% Regarding the lack of specification of frames in Sec 4.1 and 4.3: Sec 4.1 used the frame illustrated in Figure 1, while Sec 4.4 used a frame whose spanning axes of an equiangular frame, as illustrated in Figure 5. We will make this more explicit in the main text.
% }

% \david{I would be more concise: the optimal solution to objective \eqref{eq:ZCAobjective} does not depend on the choice of frame, whereas the convergence rate of Algorithm \ref{alg:online} does depend on the frame.}

3. In the case of ill-conditioned data, the authors show in Fig. 5 that while normal whitening decorrelates the data, it does so at the cost of amplifying noise. They then show and state (5C) that a modification of their method "rescales the data without amplifying noise. However, it is difficult to interpret these findings. For one, could the authors explain why rescaling the data in this case is a positive feature of their method? Secondly, since, in this scenario, we can no longer gain intuition for how well the method does by comparing it to the unit (hyper)sphere, how should we judge the performance of the algorithm? What is the optimal solution in this case, for example? As it stands, I do not understand how the outputs of the method in the ill-conditioned case indicate that the method works well vs. simply not attempting to whiten such low-rank inputs at all.

\eero{EPS: The reviewer is right about this- that section is a bit confusing.  Our framework is normative, aiming to achieve a goal of unit covariance, but this section is abruptly ad hoc in expressing the goal of not amplifying noise. One way to fix it is to state the Atick-Redlich objective, of optimizing the mutual information transmission in the presence of noise. For natural images with 1/f spectra, their solution is (approximately) a product of a whitening filter and a lowpass filter. That is, lLow frequencies are much larger than the noise so they are whitened, but high frequencies of similar or smaller amplitude than the noise are suppressed. I don't think this can be expressed in closed form, but maybe citing A-R can provide a more sound motivation?}

\mitya{I agree with Eero}

\lyndon{
Thank you for raising this concern. We will amend the text to provide further intuition and motivation for this section. We were motivated by the optimization objective of Atick \& Redlich (1992), who propose that the cells in the retina encode visual inputs by optimizing mutual information while accounting for noise. For natural images with 1/f spectra, their solution is approximately a product of a whitening filter and a lowpass filter. That is, low frequencies are much larger than the noise so they are whitened, but high frequencies of similar or smaller amplitude than the noise are suppressed. 
Our model extension outlined in Sec 4.4 naturally captures this effect by adapting to inputs whose marginal variances lie above a given threshold.
Our method is similar to (but distinct from) ideas of soft/regularized whitening, in which eigenvalues under a certain threshold are not amplified.
To provide a better quantitative measure of performance, we will rectify the spectral error to account for the inequality constraint of the non-negative whitening objective: $\sum_i \max(\lambda_i - 1, 0)^2$ where $\lambda_i$ is the ith eigenvalue of ${\bf C}_{yy}$.

% Real systems (both biological and engineered) have finite dynamic operating ranges, and an adaptively efficient system should strive to fully utilize its dynamic range while keeping in mind signal-to-noise levels. In neuroscience, several studies (e.g. Fairhall et al. 2001, Nature) have shown that biological neurons use gain modulation to rapidly (approx. 10msec) re-scale their response functions under different stimulus contexts to efficiently encode the statistics of the stimuli, with improved efficacy when adapting to high signal variance compared to low signal variance regimes.
% This difference is due to signal-to-noise ratios in high and low signal variance regimes -- it would not be optimal to amplify noise.
% Our model extension outlined in Sec 4.4 naturally captures this effect by adapting to inputs whose marginal variances lie above a given threshold.
% Our method is similar (but distinct) from ideas of soft/regularized whitening, in which eigenvalues under a certain threshold are not amplified.
}

4. The authors describe (L 332) other biologically plausible normative models that employ short-term plasticity, and then indicate (L 345) that they have focused on a different mechanism; namely, gain modulation. However, (A) they do not discuss which algorithm might perform better, an important point in judging the utility of the authors' algorithm in ML applications, and (B) they do not discuss at all which mechanism might be more plausible to explain the whitening findings in neuroscience. Nor do they propose ways by which future experiments might adjudicate between these competing hypotheses. Both of these points are especially of interest given that the performance of the present algorithm depends on the choice of W, a choice that is presumably entirely side-stepped by the methods that involve plastic, learned W. Thus, I am left wondering whether the authors' method, as conceptually interesting as I believe it is, is of interest to either the ML or neuro communities.

\eero{EPS: Another thoughtful comment from this reviewer.  

Thank you for your thoughtful review. We will revise the Intro and Discussion to include the following points to ensure our study's relevance is clear to both the neuro and ML communities.

Neuro: It's been known for nearly 100 years (Adrian, 1929) that individual neurons adjust their sensitivity (gain) adaptively, depending on recent response history. These effects are rapid, and reversible. Recent data suggest that groups of neurons seem to adapt jointly, adjusting both the amplitude of their responses, as well as their correlations.  The natural thought is that they are achieving this by adjusting the strength of their interactions (weights). Our framework provides a novel alternative: these effects can arise solely through gain changes, thereby generalizing rapid and reversible single-neuron adaptive gain modulation to the level of a neural population. 
Support for this hypothesis can come from experimental verification of the architectural requirements (reciprocally connected interneurons, with the right quantity; e.g. in the olfactory bulb), and will ultimately require careful measurement and analysis of responses and gains of neurons in a circuit during adaptation. Our revision will include precise experimental predictions that can adjudicate between our model and synaptic learning.

ML:  Whitening is one of the most basic and well-known forms of efficient signal representation, widely used in compression and channel coding. DNNs are generally not trained to whiten, although their response variances are generally normalized during training through batch normalization, and recent methods (vicREG, Bardes et al 2021) do impose global whitening properties in their objective functions. Future architectures may benefit from online, adaptive (run-time) adjustments to changing input statistics (e.g., gain-tuning, Mohan et al, NeurIPS 2021). Our proposed framework provides an unsupervised, online adaptation mechanism to prevent 'catastrophic forgetting' in neural networks during continual learning (sometimes referred to as test-time adaptation, or online fine-tuning).
}


% \david{
% Regarding the convergence rate of our model, when $W$ is a spectral frame, then we have the following:
% \begin{align*}
%     \frac{d}{dt}\|(WGW^\top)^2 - C\|^2&=2\text{tr}((WGW^\top)^2-C)(WGW^\top W\frac{dG}{dt}W^\top)\\
%     &=2\text{tr}W(G^2-\Lambda)W^\top(WG\frac{dG}{dt}W^\top)\\
%     &=2\text{tr}(G^2-\Lambda)G\text{diag}(W^\top(WGW^\top)^{-1}C(WGW^\top)^{-1}W-1)\\
%     &=2\text{tr}(G^2-\Lambda)G\text{diag}((G)^{-1}\Lambda(G)^{-1}-1)\\
%     &=2\text{tr}(G^2-\Lambda)G^{-1}(\Lambda-G^2)\\
%     &=-2\text{tr}G^{-1}(G^2-\Lambda)
% \end{align*}
% (A) Regarding our framework's relevant to the ML community, we emphasize 2 points:  \\ \\
% (B) Regarding our framework's relevant to the neuroscience community, we see gain adaptation and synaptic weight updates as complementary mechanisms. In our numerical experiments, we find that the.}

% \lyndon{
% We appreciate your thoughtful review and the points you raised about our model's relevance to ML and neuro communities.
% We would like to stress that, from a neuroscience perspective, gain modulation is a \textit{complementary} mechanism to plastic synaptic learning. Thus, pitting two algorithms (weights vs gains) against each other would not be informative because the intention of our study was not to supplant all of synaptic learning with gain modulation.

% A) Regarding our framework's relevance for the the general ML community, we feel it is important to emphasize two points: 
% 1) Whereas existing approaches to online statistical whitening boil down to synaptic learning, our study introduces a completely different and novel approach which allows pre-learned weights to remain in tact.
% To do this, we have introduced a novel symmetric matrix factorization using an arbitrary, overcomplete basis and learnable scalar components, which are amenable to being interpreted as scalar gain modulations of fixed features (Eq 8; and Appendix F).
% 2) Because gain modulation of fixed features is easily reversible, our proposed framework provides an unsupervised adaptation mechanism to prevent 'catastrophic forgetting' in neural networks during continual learning (sometimes referred to as test-time adaptation, or network online fine-tuning).
% Some recent (non-exhaustive) successful uses of reversible gain modulation of fixed pre-learned features in different ML vision applications are listed in paragraph 2 of our discussion. 

% B) We will add a more thorough discussion on which mechanism might be more plausible for whitening found in biological neural networks, including experimental predictions that could differentiate our model from existing ones. [...]
% % Mention olfactory bulb which have reciprocal connections between primary and interneurons.
% % Measured gains should increase with increase in signal input variance. This stands in contrast to classical single-neuron adaptation studies which have typically found that gains decrease with increased input variance. 

% }

\subsubsection{Limitations}
The authors discuss some practical limitations involved in their needing to pre-specify W, though, as described in Strengths and Weaknesses above, some additional information regarding these limitations would be welcome.

\lyndon{We will include additional information regarding these limitations, related to what was described in our response to point \#2, in the updated version of our paper. }

\subsection{Reviewer 3: 6(4)}

\subsubsection{Weaknesses}
A major weakness of the paper is the limited novelty of the approach. Whitening is considered to be a problem that can be easily solved, for example with ZCA, and although the approach presented here is relatively new, it should be illustrated with solid examples. The only practical application is to imagelets, which is quite limited.

\eero{We completely agree: whitening is a well-studied problem in statistics and many other fields, with well-known linear-algebraic closed-form solutions (e.g., ZCA, etc).  But the problem of \textit{online} adaptive whitening (i.e. adjusting to the statistics of changing inputs) is wide open. Adaptation is a ubiquitous property of biological neurons, and we believe it will prove important in artificial systems (e.g. with video inputs, as you mention below).  Our framework provides a step toward that goal. We'll clarify these motivations in the Introduction of the paper (see also response to R2).}

\mitya{I agree with the above response but would combine the first two sentences into one: We agree that whitening in the offline setting is an easily solved problem (e.g. with ZCA) but online adaptive whitening (i.e. adjusting to the statistics of changing inputs) is wide open. }

\lyndon{
We agree that whitening in the offline setting is an easily solved problem (e.g. with ZCA), but online adaptive whitening (i.e. adjusting to the statistics of changing inputs) is wide open. Adaptation is a ubiquitous property of biological neurons, and we believe it will prove important in artificial systems (e.g. with video inputs, as you mention below).  Our framework provides a step toward that goal. We'll clarify these motivations in the Introduction of the paper (see also response to R2).
}

Also, the introduction states that whitening is essential in some self-supervised learning algorithms, such as sparse coding - which usually uses ZCA. However, the effect of your novel algorithm on such algorithms is not evaluated, which limits the impact of the results.

\eero{EPS: this comment and the previous one indicate the reviewer is missing the main point regarding ADAPTIVE whitening - they're asking how our version of ZCA is better than the standard one.  The simple answer is that it's NOT (it's the same, from a statistical perspective).  I'd re-iterate that our method computes ZCA adaptively. As for using it as a pre-procesing step for ICA, I'd just refer them to the later response (1.3.2).}

\lyndon{

The reviewer asks whether our version of ZCA is better than standard ZCA. To be clear: from a statistical perspective, our method converges to exactly that of well-studied offline ZCA solutions. The benefit of our approach is that it enables \textit{online adaptive} whitening of inputs through a novel gain modulation mechanism, which allows pre-learned features (${\bf W}$) to remain fixed (see response to R2). This is why our examples (e.g. Fig 2, 4) emphasize whitening under changing input statistical contexts. Regarding the utility of our method for self-supervised algorithms, see \#1 below; additionally, it can also be used as a preprocessing step, as is convention for sparse coding/ICA (see our answer to your Qs below).

We have performed two additional applications of our framework, which we will include in the appendix and refer to in the main text.

1) Self-supervised online principal subspace learning. Neural feature collapse is a pervasive problem in representation learning, where several learned features redundantly collapse to a single variate of the data. We show that our unsupervised whitening framework provides a novel and effective means to prevent neural collapse during online learning.

2) We show that our online framework can be used to transform inputs with given covariance matrix to outputs with \textit{any} target covariance (i.e. not just the identity matrix), thus showing that the model has implications far beyond statistical whitening. This has implications for adaptive control systems which strive to maintain consistent output statistics under changing input statistics. For example, biological neural networks have been shown to adapt to time-varying inputs so as to homeostatically maintain a target (but not white) output covariance (Benucci et al. 2013).
}

\subsubsection{Questions}

Related to the weakness pointed above, could you scale your framework to bigger images, or even to video streams? The equations you propose seem to quite naturally extend to that framework, yet the convergence of the solution should be checked.

\lyndon{Yes, our framework can scale to bigger images and video streams. Due to time constraints of the rebuttal period, we could not procure \& prepare a high-res video dataset. However, we'd like to emphasize two points. 1) The theoretical foundations of our method provide asymptotic guarantees on algorithm performance. Namely, Appendix H. ('Whitening spatially local neighborhoods') shows that using our local whitening procedure with convolutional weights produces a drastic reduction in asymptotic worst-case complexity $\mathcal{O}(N^2) \rightarrow \mathcal{O}(N)$, which therefore makes our method practically feasible for whitening high-resolution images. 2) The imagelets (Fig 5) are a video dataset where each imagelet is a frame sequentially drawn using a Gaussian random walk, and therefore validates that our convolutional framework can already operate on video data. 
}

I did not see in the paper an interpretation of the factor $g_i$ with respect to the projection of on $x$ and $w_i$,  notably by giving a closed form solution to Eq 10.

\lyndon{
We will revise the text to include an intuitive statement about $g$ and its relationship to x and $w_i$. We have already included the closed-form steady-state solution to ${\bf g}$ as a function of ${\bf x}$ and ${\bf W}$ in Appendix F, and will emphasize it in the revision. Intuitively, when the marginal variance of the joint primary neuron activities is higher than 1 along an interneuron's projection axis, the interneuron will increase its gain to suppress joint primary neuron activities along that axis; conversely, if marginal variance is lower than 1, it will decrease its gain to allow joint activity variance to grow along that axis. What is remarkable is that despite all interneurons adjusting their gains independently from one another, the interneuron responses act \textit{in concert} to ultimately whiten the joint primary neuron activities. 
}

Could you directly integrate your formulation in a sparse coding scheme?

\lyndon{
Yes, in fact Section 4.3 ('Implicit gating via gain modulation') is an example of how our framework ties in with sparse coding concepts. Specifically, assuming there are multiple contexts (pre-learned over long time scales) embedded in the fixed frame ${\bf W}$, our derived gain modulation mechanism can sparsely select the relevant frame vectors \textit{without} modification of the objective or network. For an explicit constraint similar to previous sparse coding approaches, it is possible to add a tuneable $\ell_1$ penalty on the gains directly to the objective, or the interneuron activities. We have conducted preliminary experiments using this approach and have confirmed its ability to whiten using a sparse set of available interneurons. We will re-write the text in this section to make this connection more clear.
}

\subsubsection{Limitations}

One limitation of the paper is that the literature review is quite limited to very recent papers. I was quite surprised not to see a paper by J. Atick cited (e.g. "What does the retina know about natural scenes?"), or several papers on sparse coding that find neurally plausible solutions to the problem of finding the gain of neurons.

\lyndon{
Thank you for the suggestion - we should be citing a number of classic comp neuro papers on coding efficiency that provide context and background for our approach, including Atick \& Redlich 1992; Barlow \& Foldiak, 1992; Olshausen \& Field, 1996; Bell \& Sejnowski, 1997; Schwartz \& Simoncelli, 2000.
%PCA w/ Linsker; brenner; fairhall; matteo}). 
}

